From SuperBIT to GigaBIT: Informing next-generation balloon-borne telescope design with Fine Guidance System flight data

The Super-pressure Balloon-borne Imaging Telescope (SuperBIT) is a near-diffraction-limited 0.5m telescope that launched via NASA's super-pressure balloon technology on April 16, 2023. SuperBIT achieved precise pointing control through the use of three nested frames in conjunction with an optical Fine Guidance System (FGS), resulting in an average image stability of 0.055" over 300-second exposures. The SuperBIT FGS includes a tip-tilt fast-steering mirror that corrects for jitter on a pair of focal plane star cameras. In this paper, we leverage the empirical data from SuperBIT's successful 45-night stratospheric mission to inform the FGS design for the next-generation balloon-borne telescope. The Gigapixel Balloon-borne Imaging Telescope (GigaBIT) is designed to be a 1.35m wide-field, high resolution imaging telescope, with specifications to extend the scale and capabilities beyond those of its predecessor SuperBIT. A description and analysis of the SuperBIT FGS will be presented along with methodologies for extrapolating this data to enhance GigaBIT's FGS design and fine pointing control algorithm. We employ a systems engineering approach to outline and formalize the design constraints and specifications for GigaBIT's FGS. GigaBIT, building on the SuperBIT legacy, is set to enhance high-resolution astronomical imaging, marking a significant advancement in the field of balloon-borne telescopes.

==> figures/Algo.tex <==


\begin{algorithm}[H]
    \caption{$\vert$ Ray-Tracing Intersect Function}
    \label{algo1} 
    \begin{algorithmic}[1] 
    
    \Require $\theta,\ \phi,\ \alpha,\ \beta,\ \textbf{p}_0,\ \textbf{p}_r,\ \textbf{r}_i$  --  Control and mounting angles, Points on surface and ray, Incident ray 
    
    \Ensure $\textbf{p}_{si},\ \textbf{r}_r$  --  Point of surface intersection, Reflected ray 
    
    \vspace{8pt}
    
    \Function{reflection}{$\theta,\ \phi,\ \alpha,\ \beta,\ \textbf{p}_0,\ \textbf{p}_r,\ \textbf{r}_i$}
    
    \Statex {\small \texttt{ // Define surface normal in body frame}}

    \vspace{5pt}

    \State $\textbf{C}_{b,m}\ \gets \ \begin{bmatrix} \cos\beta\cos\alpha & -\sin\beta & \minus\cos\beta\sin\alpha\\ \sin\beta\cos\alpha & \cos\beta & \minus\sin\beta\sin\alpha\\ \sin\alpha & 0 & \cos\alpha \end{bmatrix}$

    \vspace{5pt}

    \State $\textbf{n}_m\ \gets \ \begin{bmatrix} \cos\theta\cos\phi\\ \cos\theta\sin\phi\\ \minus \sin\theta\cos\phi\\ \end{bmatrix}$

    \vspace{5pt}

    \State $\textbf{n}_b\ \gets \ \textbf{C}_{b,m}\ \textbf{n}_m$

    \vspace{4pt}

    
    \Statex {\small \texttt{// Define intersection and vector reflection}}

    \vspace{4pt}

    \State $s_i\ \gets \   \begin{matrix} \frac{\textbf{n}_b^\intercal(\textbf{p}_0 \minus \textbf{p}_r)}{\textbf{n}_b^\intercal \textbf{r}_i} \end{matrix}$

    \vspace{3pt}

    \State $\textbf{T}\ \gets \ \textbf{1} \ \minus\ 2 \textbf{n}_b \textbf{n}_b^\intercal$

    \vspace{1pt}

    \State $\textbf{p}_{si}\ \gets \ s_i \textbf{r}_i + \textbf{p}_r$

    \vspace{1pt}

    \State $\textbf{r}_r\ \gets \ \textbf{T}\ \textbf{r}_i$

    \vspace{1pt}
    
    \State\textbf{return} $\ \textbf{p}_{si},\ \textbf{r}_r$  

    \vspace{1pt}
    
\EndFunction
\end{algorithmic} \end{algorithm}
